Certified Symmetry and Dominance Breaking for Combinatorial Optimisation

Symmetry and dominance breaking can be crucial for solving hard combinatorial search and optimisation problems, but the correctness of these techniques sometimes relies on subtle arguments. For this reason, it is desirable to produce efficient, machine-verifiable certificates that solutions have been computed correctly. Building on the cutting planes proof system, we develop a certification method for optimisation problems in which symmetry and dominance breaking are easily expressible. Our experimental evaluation demonstrates that we can efficiently verify fully general symmetry breaking in Boolean satisfiability (SAT) solving, thus providing, for the first time, a unified method to certify a range of advanced SAT techniques that also includes XOR and cardinality reasoning. In addition, we apply our method to maximum clique solving and constraint programming as a proof of concept that the approach applies to a wider range of combinatorial problems.

==> applications-preamble.tex <==
%!TEX root = CertifiedSymmetryAndDominanceBreakingForCombinatorialOptimisation_JournalExtension.tex


\section{Applications}\label{sec:applications}

We now exhibit three applications that have
not previously
%%% Avoid repetition -JN
%   supported
admitted
%%% Important to stress that efficiency is key --- otherwise it has
%%% been doable, no? -JN 
efficient
certification, and demonstrate that our  new method
%%% Varying the language (in view of edits above) -JN
%   can support efficient proof logging in each case.
can support simple, practical  proof logging in each case.
%%% "proof logging capabilities" sounds a bit strange --- attempting a
%%% rewrite -JN
We first show that, by
%   adding proof logging capabilities to the \breakid tool for SAT
enhancing the \breakid tool for SAT
%%% When reading here I found myself missing the reference. Imagine a
%%% reader that skips right to the applications section and has no
%%% clue what BreakID is... -JN
solving~\cite{DBBD16ImprovedStatic} with \veripb proof logging, 
we can cover the entire solving toolchain when symmetries are
involved. We then revisit the Crystal Maze example from the
introduction. 
%   Finally, we discuss how to handle both dominance and optimisation in a
%   maximum clique solver.
Finally, we discuss how \domrulelong can be used 
to support vertex domination reasoning in a 
maximum clique solver.
%%%
%%% Zenodo reference here! -JNF
%%%
\textrefzenodo

%%%
%%% No really strong opinions here, it seems, so commenting out for now -JN
%%%
%   
%   \jncomment{Do we want to mention explicitly
%   ``both dominance \textbf{and optimisation}'' for max clique?
%   }
%   \bbcomment{No strong opinion on whether it should be said \emph{here}. }
%   
%   \jncomment{Proposing new version avoiding getting into details.}
%   


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "justified_sym_and_dom"
%%% End:



==> theorems.tex <==

\usepackage{amsthm}
\usepackage{thmtools}

\declaretheorem[style=plain,	name=Theorem,		numberwithin=section]{thm}
\declaretheorem[style=plain,	name=Theorem,		numberlike=thm]{theorem}
\declaretheorem[style=plain,	name=Proposition,	numberlike=thm]{prop}
\declaretheorem[style=plain,	name=Proposition,	numberlike=thm]{proposition}
\declaretheorem[style=plain,	name=Lemma,		numberlike=thm]{lem}
\declaretheorem[style=plain,	name=Lemma,		numberlike=thm]{lemma}
\declaretheorem[style=plain,	name=Lemma,		numbered=no]   {lem*}
\declaretheorem[style=plain,	name=Corollary,		numberlike=thm]{cor}
\declaretheorem[style=plain,	name=Corollary,		numberlike=thm]{corollary}
\declaretheorem[style=plain,	name=Conjecture,	numberlike=thm]{conjecture}

\declaretheorem[style=definition,	name=Definition,	numberlike=thm]{definition}
\declaretheorem[style=definition,	name=Definition,	numberlike=thm]{defn}
\declaretheorem[style=definition,	qed=$\blacktriangle$,	numberlike=thm]{example}
\declaretheorem[style=definition,	qed=$\blacktriangle$,	numberlike=thm]{ex}
\declaretheorem[style=definition,	qed=$\blacktriangle$,	numbered=no]{ex*}

\declaretheorem[style=remark,		name=Notation,		numberlike=thm]{nota}
\declaretheorem[style=remark,	name=Notation,		numbered=no]{nota*}
\declaretheorem[style=remark,	qed=$\blacktriangle$,	name=Note,		numberlike=thm]{note}
\declaretheorem[style=remark,	qed=$\blacktriangle$,	name=Note,		numbered=no]{note*}
\declaretheorem[style=remark,	qed=$\blacktriangle$,	name=Remark,		numberlike=thm]{remark}

